FhGenie: A Custom, Confidentiality-preserving Chat AI for Corporate and Scientific Use

Since OpenAI's release of ChatGPT, generative AI has received significant attention across various domains. These AI-based chat systems have the potential to enhance the productivity of knowledge workers in diverse tasks. However, the use of free public services poses a risk of data leakage, as service providers may exploit user input for additional training and optimization without clear boundaries. Even subscription-based alternatives sometimes lack transparency in handling user data. To address these concerns and enable Fraunhofer staff to leverage this technology while ensuring confidentiality, we have designed and developed a customized chat AI called FhGenie (genie being a reference to a helpful spirit). Within few days of its release, thousands of Fraunhofer employees started using this service. As pioneers in implementing such a system, many other organizations have followed suit. Our solution builds upon commercial large language models (LLMs), which we have carefully integrated into our system to meet our specific requirements and compliance constraints, including confidentiality and GDPR. In this paper, we share detailed insights into the architectural considerations, design, implementation, and subsequent updates of FhGenie. Additionally, we discuss challenges, observations, and the core lessons learned from its productive usage.

==> section_legal_pub_sector.tex <==
% tmur
\section{Artificial Intelligence and Digitization in the Public Sector}

\tmur{work in progress...}

The integration of information technology in the public sector, along with its legal ramifications, constitutes a distinct field of study, traceable for decades in the past \cite{BrinkmannKuhlmann1990} \cite{Reinermann1997}.

As IT continues to permeate public services, regulatory compliance 
challenges remain constant, notably with the recent emergence of artificial intelligence.

Any digitally outsourced business process holds potential data privacy related risks by its distributed nature; the AI case 
with the GPT4 technology being unique in its performance at the given time, 
questions organizations' competitiveness not integrating with it. (sources..?)

Research topics focus here beyond literature reviews \cite{Fischer_etal_2021} and .. on ... ethical discussions around AI.

%  [politically correct statements about required efforts go here ]
Looking forward, suggested research agenda topics, specifically (...) appear relevant in our context (because ... ), and further scientific findings in this research field could foster the implementation and digitization of the internal legal validation processes.



==> source_collection.tex <==

Entry level/Discussion

"You do not need hosted LLMs, don't you?" by Savvov (8/2023) on Medium.com
https://betterprogramming.pub/you-dont-need-hosted-llms-do-you-1160b2520526
Quote: "For lower usage in the 10,000’s requests per day range, OpenAI API works out cheaper than using self-hosted LLMs."
=> 10K*30=300K / month -> approx. 200.000 questions per month in Fraunofer - we are moving to there, as it seems?

















Wissenswert am Rande /geistesw. Kontext: interessant Bezüge auf Hermeneutik im Sinne des hermen. Kreis der Erkenntnis
durch neue Inerpretationen, was das überhaupt alles bedeuten kann, wenn das "Gegenüber" ein GPT/LLM System ist.
https://en.wikipedia.org/wiki/Hermeneutic_circle
https://www.mdpi.com/2813-0324/8/1/94

